Linear systems solvers - recent developments and implications for lattice computations

We review the numerical analysis' understanding of Krylov subspace methods for solving (non-hermitian) systems of equations and discuss its implications for lattice gauge theory computations using the example of the Wilson fermion matrix. Our thesis is that mature methods like QMR, BiCGStab or restarted GMRES are close to optimal for the Wilson fermion matrix. Consequently, preconditioning appears to be the crucial issue for further improvements.

==> maths.tex <==
%auto-ignore
% --- standard sets -----------------------------------------------------------

% --- serif version ---

\newcommand{\mathC}{\mbox{\rm \hspace*{0.2em}\rule[0.03em]{0.035em}{0.59em}\hspace*{-0.235em}C}}
\newcommand{\mathN}{\mbox{\rm I\hspace*{-0.21em}N}}
\newcommand{\mathQ}{\mbox{\rm \hspace*{0.2em}\rule[0.03em]{0.035em}{0.59em}\hspace*{-0.235em}Q}}
\newcommand{\mathR}{\mbox{\rm I\hspace*{-0.21em}R}}
\newcommand{\mathZ}{\mbox{\sf Z\hspace*{-0.46em}Z}}

% --- sans serif version ---

\newcommand{\MathC}{\mbox{\sf \hspace*{0.25em}\rule[0.05em]{0.035em}{0.59em}\hspace*{-0.285em}C}}
\newcommand{\MathN}{\mbox{\sf I\hspace*{-0.15em}N}}
\newcommand{\MathQ}{\mbox{\sf \hspace*{0.2em}\rule[0.05em]{0.035em}{0.59em}\hspace*{-0.235em}Q}}
\newcommand{\MathR}{\mbox{\sf I\hspace*{-0.12em}R}}
\newcommand{\MathZ}{\mbox{\sf Z\hspace*{-0.46em}Z}}


